Neural Bregman Divergences for Distance Learning

Many metric learning tasks, such as triplet learning, nearest neighbor retrieval, and visualization, are treated primarily as embedding tasks where the ultimate metric is some variant of the Euclidean distance (e.g., cosine or Mahalanobis), and the algorithm must learn to embed points into the pre-chosen space. The study of non-Euclidean geometries is often not explored, which we believe is due to a lack of tools for learning non-Euclidean measures of distance. Recent work has shown that Bregman divergences can be learned from data, opening a promising approach to learning asymmetric distances. We propose a new approach to learning arbitrary Bergman divergences in a differentiable manner via input convex neural networks and show that it overcomes significant limitations of previous works. We also demonstrate that our method more faithfully learns divergences over a set of both new and previously studied tasks, including asymmetric regression, ranking, and clustering. Our tests further extend to known asymmetric, but non-Bregman tasks, where our method still performs competitively despite misspecification, showing the general utility of our approach for asymmetric learning.

==> tables/deep_div_table.tex <==
\begin{tabular}{llrrrr}
\toprule
     &     &  knn@1 &  knn@5 &  prec@10 &  map@10 \\
dataset & model &        &        &          &         \\
\midrule
cifar10 & deep-div &  0.517 &  0.566 &    0.532 &   0.611 \\
     & euclidean &  0.819 &  0.823 &    0.819 &   0.831 \\
     & nbd &  0.820 &  0.823 &    0.819 &   0.830 \\
fmnist & deep-div &  0.496 &  0.497 &    0.477 &   0.551 \\
     & euclidean &  0.903 &  0.909 &    0.903 &   0.913 \\
     & nbd &  0.904 &  0.911 &    0.904 &   0.914 \\
stl10 & deep-div &  0.198 &  0.211 &    0.195 &   0.291 \\
     & euclidean &  0.574 &  0.601 &    0.568 &   0.629 \\
     & nbd &  0.548 &  0.572 &    0.546 &   0.597 \\
svhn & deep-div &  0.079 &  0.184 &    0.121 &   0.244 \\
     & euclidean &  0.952 &  0.954 &    0.953 &   0.956 \\
     & nbd &  0.951 &  0.952 &    0.951 &   0.954 \\
\bottomrule
\end{tabular}


==> tables/ranking_table_full.tex <==
\begin{tabular}{llllll}
\toprule
     &          &         final_map &         final_auc &      final_purity &        final_rand \\
dataset & model &                   &                   &                   &                   \\
\midrule
\multirow{7}{*}{abalone} & Deep-div &  $0.281_{\ 0.01}$ &  $0.645_{\ 0.02}$ &  $0.377_{\ 0.02}$ &   $0.66_{\ 0.04}$ \\
     & deepnorm &  $0.312_{\ 0.01}$ &  $0.672_{\ 0.01}$ &  $0.426_{\ 0.02}$ &  $0.745_{\ 0.01}$ \\
     & Euclidean &  $0.301_{\ 0.01}$ &  $0.666_{\ 0.01}$ &  $0.422_{\ 0.03}$ &   $0.75_{\ 0.01}$ \\
     & Mahalanobis &   $0.31_{\ 0.01}$ &  $0.677_{\ 0.01}$ &  $0.419_{\ 0.02}$ &   $0.75_{\ 0.01}$ \\
     & NBD &  $0.316_{\ 0.01}$ &  $0.682_{\ 0.01}$ &  $0.432_{\ 0.03}$ &   $0.75_{\ 0.01}$ \\
     & PBDL &  $0.307_{\ 0.01}$ &  $0.659_{\ 0.01}$ &  $0.386_{\ 0.02}$ &  $0.735_{\ 0.02}$ \\
     & widenorm &  $0.315_{\ 0.01}$ &  $0.681_{\ 0.01}$ &  $0.255_{\ 0.02}$ &  $0.188_{\ 0.01}$ \\
\cline{1-6}
\multirow{7}{*}{balance-scale} & Deep-div &  $0.804_{\ 0.03}$ &  $0.859_{\ 0.02}$ &  $0.869_{\ 0.02}$ &  $0.828_{\ 0.03}$ \\
     & deepnorm &  $0.822_{\ 0.01}$ &  $0.856_{\ 0.01}$ &  $0.813_{\ 0.06}$ &  $0.723_{\ 0.06}$ \\
     & Euclidean &  $0.611_{\ 0.01}$ &  $0.666_{\ 0.01}$ &  $0.633_{\ 0.06}$ &  $0.568_{\ 0.04}$ \\
     & Mahalanobis &  $0.822_{\ 0.01}$ &  $0.854_{\ 0.01}$ &  $0.851_{\ 0.06}$ &  $0.761_{\ 0.05}$ \\
     & NBD &  $0.887_{\ 0.01}$ &  $0.915_{\ 0.01}$ &  $0.898_{\ 0.02}$ &  $0.872_{\ 0.03}$ \\
     & PBDL &  $0.836_{\ 0.02}$ &  $0.855_{\ 0.02}$ &  $0.872_{\ 0.02}$ &  $0.814_{\ 0.03}$ \\
     & widenorm &   $0.82_{\ 0.01}$ &  $0.855_{\ 0.01}$ &  $0.839_{\ 0.06}$ &  $0.749_{\ 0.06}$ \\
\cline{1-6}
\multirow{7}{*}{car} & Deep-div &  $0.787_{\ 0.01}$ &  $0.757_{\ 0.01}$ &  $0.852_{\ 0.04}$ &   $0.75_{\ 0.04}$ \\
     & deepnorm &   $0.79_{\ 0.01}$ &  $0.752_{\ 0.01}$ &  $0.781_{\ 0.03}$ &  $0.658_{\ 0.03}$ \\
     & Euclidean &   $0.681_{\ 0.0}$ &   $0.589_{\ 0.0}$ &  $0.704_{\ 0.02}$ &  $0.523_{\ 0.03}$ \\
     & Mahalanobis &  $0.787_{\ 0.01}$ &  $0.752_{\ 0.01}$ &  $0.778_{\ 0.02}$ &  $0.654_{\ 0.03}$ \\
     & NBD &   $0.82_{\ 0.01}$ &  $0.803_{\ 0.01}$ &   $0.86_{\ 0.01}$ &  $0.758_{\ 0.02}$ \\
     & PBDL &  $0.798_{\ 0.01}$ &  $0.775_{\ 0.01}$ &  $0.854_{\ 0.01}$ &   $0.75_{\ 0.02}$ \\
     & widenorm &  $0.793_{\ 0.01}$ &  $0.782_{\ 0.01}$ &  $0.834_{\ 0.03}$ &  $0.723_{\ 0.03}$ \\
\cline{1-6}
\multirow{7}{*}{iris} & Deep-div &  $0.945_{\ 0.03}$ &  $0.967_{\ 0.02}$ &  $0.811_{\ 0.16}$ &   $0.82_{\ 0.16}$ \\
     & deepnorm &  $0.949_{\ 0.02}$ &  $0.975_{\ 0.01}$ &  $0.943_{\ 0.09}$ &   $0.94_{\ 0.08}$ \\
     & Euclidean &  $0.827_{\ 0.02}$ &  $0.897_{\ 0.01}$ &   $0.82_{\ 0.07}$ &  $0.828_{\ 0.05}$ \\
     & Mahalanobis &  $0.946_{\ 0.03}$ &  $0.973_{\ 0.01}$ &  $0.884_{\ 0.12}$ &  $0.879_{\ 0.11}$ \\
     & NBD &  $0.957_{\ 0.02}$ &  $0.977_{\ 0.01}$ &   $0.909_{\ 0.1}$ &   $0.902_{\ 0.1}$ \\
     & PBDL &  $0.943_{\ 0.03}$ &  $0.967_{\ 0.02}$ &  $0.889_{\ 0.14}$ &  $0.888_{\ 0.13}$ \\
     & widenorm &  $0.948_{\ 0.02}$ &  $0.974_{\ 0.01}$ &  $0.912_{\ 0.11}$ &   $0.911_{\ 0.1}$ \\
\cline{1-6}
\multirow{7}{*}{transfusion} & Deep-div &  $0.648_{\ 0.01}$ &  $0.525_{\ 0.02}$ &  $0.756_{\ 0.03}$ &  $0.621_{\ 0.04}$ \\
     & deepnorm &  $0.681_{\ 0.01}$ &  $0.569_{\ 0.01}$ &  $0.749_{\ 0.03}$ &  $0.542_{\ 0.04}$ \\
     & Euclidean &  $0.666_{\ 0.01}$ &  $0.536_{\ 0.01}$ &  $0.748_{\ 0.03}$ &  $0.563_{\ 0.04}$ \\
     & Mahalanobis &   $0.68_{\ 0.01}$ &   $0.57_{\ 0.01}$ &   $0.75_{\ 0.03}$ &  $0.543_{\ 0.05}$ \\
     & NBD &  $0.695_{\ 0.01}$ &  $0.603_{\ 0.01}$ &  $0.756_{\ 0.03}$ &    $0.6_{\ 0.04}$ \\
     & PBDL &  $0.637_{\ 0.01}$ &  $0.504_{\ 0.01}$ &  $0.748_{\ 0.03}$ &  $0.622_{\ 0.03}$ \\
     & widenorm &  $0.715_{\ 0.02}$ &   $0.63_{\ 0.02}$ &  $0.765_{\ 0.03}$ &  $0.639_{\ 0.03}$ \\
\cline{1-6}
\multirow{7}{*}{wine} & Deep-div &  $0.983_{\ 0.02}$ &  $0.987_{\ 0.01}$ &  $0.953_{\ 0.08}$ &  $0.947_{\ 0.08}$ \\
     & deepnorm &  $0.953_{\ 0.02}$ &  $0.971_{\ 0.01}$ &   $0.929_{\ 0.1}$ &  $0.924_{\ 0.09}$ \\
     & Euclidean &  $0.844_{\ 0.02}$ &  $0.884_{\ 0.02}$ &  $0.902_{\ 0.07}$ &  $0.887_{\ 0.06}$ \\
     & Mahalanobis &  $0.949_{\ 0.02}$ &   $0.97_{\ 0.01}$ &   $0.944_{\ 0.1}$ &   $0.94_{\ 0.09}$ \\
     & NBD &  $0.969_{\ 0.02}$ &   $0.98_{\ 0.01}$ &   $0.96_{\ 0.05}$ &  $0.948_{\ 0.06}$ \\
     & PBDL &  $0.978_{\ 0.02}$ &  $0.982_{\ 0.01}$ &   $0.82_{\ 0.14}$ &  $0.823_{\ 0.12}$ \\
     & widenorm &  $0.955_{\ 0.02}$ &  $0.973_{\ 0.01}$ &   $0.93_{\ 0.12}$ &   $0.929_{\ 0.1}$ \\
\bottomrule
\end{tabular}

==> tables/ranking_table_with_stdev.tex <==

\begin{table}
\centering
\begin{tabular}{llcccc}
\toprule
     &      &         MAP &         AUC &      Purity &        Rand Index \\
Dataset & Model &                   &                   &                   &                   \\
\midrule
\multirow{5}{*}{abalone} & Deep-div &  $0.281_{\ 0.01}$ &  $0.645_{\ 0.02}$ &  $0.377_{\ 0.02}$ &   $0.660_{\ 0.04}$ \\
     & Euclidean &  $0.301_{\ 0.01}$ &  $0.666_{\ 0.01}$ &  $0.422_{\ 0.03}$ &   $\mathbf{0.750}_{\ 0.01}$ \\
     & Mahalanobis &   $0.310_{\ 0.01}$ &  $0.677_{\ 0.01}$ &  $0.419_{\ 0.02}$ &   $\mathbf{0.750}_{\ 0.01}$ \\
     & NBD &  $\mathbf{0.316}_{\ 0.01}$ &  $\mathbf{0.682}_{\ 0.01}$ &  $\mathbf{0.432}_{\ 0.03}$ &   $\mathbf{0.750}_{\ 0.01}$ \\
     & PBDL &  $0.307_{\ 0.01}$ &  $0.659_{\ 0.01}$ &  $0.386_{\ 0.02}$ &  $0.735_{\ 0.02}$ \\
\cline{1-6}
\multirow{5}{*}{balance-scale} & Deep-div &  $0.804_{\ 0.03}$ &  $0.859_{\ 0.02}$ &  $0.869_{\ 0.02}$ &  $0.828_{\ 0.03}$ \\
     & Euclidean &  $0.611_{\ 0.01}$ &  $0.666_{\ 0.01}$ &  $0.633_{\ 0.06}$ &  $0.568_{\ 0.04}$ \\
     & Mahalanobis &  $0.822_{\ 0.01}$ &  $0.854_{\ 0.01}$ &  $0.851_{\ 0.06}$ &  $0.761_{\ 0.05}$ \\
     & NBD &  $\mathbf{0.887}_{\ 0.01}$ &  $\mathbf{0.915}_{\ 0.01}$ &  $\mathbf{0.898}_{\ 0.02}$ &  $\mathbf{0.872}_{\ 0.03}$ \\
     & PBDL &  $0.836_{\ 0.02}$ &  $0.855_{\ 0.02}$ &  $0.872_{\ 0.02}$ &  $0.814_{\ 0.03}$ \\
\cline{1-6}
\multirow{5}{*}{car} & Deep-div &  $0.787_{\ 0.01}$ &  $0.757_{\ 0.01}$ &  $0.852_{\ 0.04}$ &   $0.750_{\ 0.04}$ \\
     & Euclidean &   $0.681_{\ 0.00}$ &   $0.589_{\ 0.00}$ &  $0.704_{\ 0.02}$ &  $0.523_{\ 0.03}$ \\
     & Mahalanobis &  $0.787_{\ 0.01}$ &  $0.752_{\ 0.01}$ &  $0.778_{\ 0.02}$ &  $0.654_{\ 0.03}$ \\
     & NBD &   $\mathbf{0.820}_{\ 0.01}$ &  $\mathbf{0.803}_{\ 0.01}$ &   $\mathbf{0.860}_{\ 0.01}$ &  $\mathbf{0.758}_{\ 0.02}$ \\
     & PBDL &  $0.798_{\ 0.01}$ &  $0.775_{\ 0.01}$ &  $0.854_{\ 0.01}$ &   $0.750_{\ 0.02}$ \\
\cline{1-6}
\multirow{5}{*}{iris} & Deep-div &  $0.945_{\ 0.03}$ &  $0.967_{\ 0.02}$ &  $0.811_{\ 0.16}$ &   $0.820_{\ 0.16}$ \\
     & Euclidean &  $0.827_{\ 0.02}$ &  $0.897_{\ 0.01}$ &   $0.820_{\ 0.07}$ &  $0.828_{\ 0.05}$ \\
     & Mahalanobis &  $0.946_{\ 0.03}$ &  $0.973_{\ 0.01}$ &  $0.884_{\ 0.12}$ &  $0.879_{\ 0.11}$ \\
     & NBD &  $\mathbf{0.957}_{\ 0.02}$ &  $\mathbf{0.977}_{\ 0.01}$ &   $\mathbf{0.909}_{\ 0.10}$ &   $\mathbf{0.902}_{\ 0.10}$ \\
     & PBDL &  $0.943_{\ 0.03}$ &  $0.967_{\ 0.02}$ &  $0.889_{\ 0.14}$ &  $0.888_{\ 0.13}$ \\
\cline{1-6}
\multirow{5}{*}{transfusion} & Deep-div &  $0.648_{\ 0.01}$ &  $0.525_{\ 0.02}$ &  $\mathbf{0.756}_{\ 0.03}$ &  $0.621_{\ 0.04}$ \\
     & Euclidean &  $0.666_{\ 0.01}$ &  $0.536_{\ 0.01}$ &  $0.748_{\ 0.03}$ &  $0.563_{\ 0.04}$ \\
     & Mahalanobis &   $0.680_{\ 0.01}$ &   $0.570_{\ 0.01}$ &   $0.750_{\ 0.03}$ &  $0.543_{\ 0.05}$ \\
     & NBD &  $\mathbf{0.695}_{\ 0.01}$ &  $\mathbf{0.603}_{\ 0.01}$ &  $\mathbf{0.756}_{\ 0.03}$ &    $0.600_{\ 0.04}$ \\
     & PBDL &  $0.637_{\ 0.01}$ &  $0.504_{\ 0.01}$ &  $0.748_{\ 0.03}$ &  $\mathbf{0.622}_{\ 0.03}$ \\
\cline{1-6}
\multirow{5}{*}{wine} & Deep-div &  $\mathbf{0.983}_{\ 0.02}$ &  $\mathbf{0.987}_{\ 0.01}$ &  $0.953_{\ 0.08}$ &  $0.947_{\ 0.08}$ \\
     & Euclidean &  $0.844_{\ 0.02}$ &  $0.884_{\ 0.02}$ &  $0.902_{\ 0.07}$ &  $0.887_{\ 0.06}$ \\
     & Mahalanobis &  $0.949_{\ 0.02}$ &   $0.970_{\ 0.01}$ &   $0.944_{\ 0.10}$ &   $0.940_{\ 0.09}$ \\
     & NBD &  $0.969_{\ 0.02}$ &   $0.980_{\ 0.01}$ &   $\mathbf{0.960}_{\ 0.05}$ &  $\mathbf{0.948}_{\ 0.06}$ \\
     & PBDL &  $0.978_{\ 0.02}$ &  $0.982_{\ 0.01}$ &   $0.820_{\ 0.14}$ &  $0.823_{\ 0.12}$ \\
\bottomrule
\end{tabular}
    \caption{Across several real datasets, a learned Bregman divergence is superior to Euclidean or Mahalanobis metrics for downstream ranking (MAP, AUC) and clustering (Purity, Rand Index) tasks. Furthermore, our approach \bregman consistently outperforms the prior Bregman learning approaches, Deep-div and PBDL, on most datasets. MAP = mean average precision, AUC = area under curve}
    \label{tab:ranking}
\end{table}

